Class based Influence Functions for Error Detection

Influence functions (IFs) are a powerful tool for detecting anomalous examples in large scale datasets. However, they are unstable when applied to deep networks. In this paper, we provide an explanation for the instability of IFs and develop a solution to this problem. We show that IFs are unreliable when the two data points belong to two different classes. Our solution leverages class information to improve the stability of IFs. Extensive experiments show that our modification significantly improves the performance and stability of IFs while incurring no additional computational cost.

==> sections/introduction_eacl.tex <==
\section{Introduction}
\label{sec:intro}
Influence function (IF) \cite{koh2017understanding} is an instance-based approach to understanding black-box predictors, especially deep neural networks.
Different from the feature-based approach, which identifies parts of the input that are responsible for the model's prediction, instance-based approach identifies which inputs are the most influential to the model's prediction.
When its assumptions are (approximately) satisfied, IF gives a reasonable estimate of the influence of a data point on another data point.
This capability allows IF to detect harmful data points - data points that have a negative influence on other data points.
IF is a powerful tool for detecting adversarial \cite{cohen2020detecting}, poisonous \cite{koh2017understanding, cina2021backdoor}, and erroneous \cite{dau2022towards} examples.
Correcting or removing anomalous examples from the training data improves the performance and robustness of models trained on such data.

The success of IF has inspired a series of follow up works on efficient influence estimation \cite{charpiat2019input, khanna2019interpreting, barshan2020relatif, pruthi2020estimating}.
For brevity, we call IF and its variants influence functions (IFs).
\citet{basu2021influence} empirically observed that IFs are unstable especially when they are applied to deep networks. %\citet{anonymous2022large} experimentally showed that when a deep network converges, most data points are independent.
%Therefore, the influence of a data point on another random data point is very subtle and hard to predict.
In Sec.~\ref{sec:method}, we provide a deeper analysis with both empirical and theoretical explanation of the phenomenon.
We show that IFs are very noisy when the two data points are in different classes, but IFs become much more stable when the two data points are in the same class.
%Our analysis sheds light on the behavior of IFs.

Motivated by our analysis, we propose class-based influence functions (IFs-class), a variant of IFs that use class information to reduce the noise in influence estimation.
Compared to IFs, IFs-class are much more stable and performant while having the same computational complexity (Sec.~\ref{sec:method},  \ref{sec:exp}).
Our improved IFs can be used in classification problems and can be easily extended to sequential classification problems such as Named Entity Recognition (NER).
%In this paper, we focus on the application of IFs and IFs-class in the error detection problem but 
%we note that they can be used in other anomalous data detection algorithms.

Our contributions include
\begin{enumerate}
\item An explanation of the instability of IFs.
Our analysis sheds light on the behavior of IFs and helps the development of better IFs.
\item A stable, high performance variant of IFs that can be used to develop better anomalous data detection algorithms.
\end{enumerate}



==> sections/related_eacl.tex <==
\section{Background and Related work}
\label{sec:related}
% Named Entity Recognition via Noise Aware Training Mechanism with Data Filter
We define the notations used in this paper.
Let $\mathbf{z} = (\mathbf{x}, \mathbf{y})$ be a data point, where $\mathbf{x} \in \mathcal{X}$ is the input, $\mathbf{y} \in \mathcal{Y}$ is the target output;
$\mathcal{Z} = \left\lbrace \mathbf{z}^{(i)} \right\rbrace_{i = 1}^n$ be a dataset of $n$ data points; 
$\mathcal{Z}_{-i} = \mathcal{Z} \backslash \mathbf{z}^{(i)}$ be the dataset $\mathcal{Z}$ with $\mathbf{z}^{(i)}$ removed;
$f_\mathbf{\bm{\theta}}: \mathcal{X} \rightarrow \mathcal{Y}$  be a model with parameter $\bm \theta$;
$\mathcal{L}_{\mathcal{Z}, \bm \theta} = \frac{1}{n} \sum_{i = 1}^n \ell(f_{{\bm{\theta}}}(\mathbf{x}^{(i)}), \mathbf{y}^{(i)}) =\frac{1}{n} \sum_{i = 1}^n \ell(\mathbf{z}^{(i)}; \bm \theta)$ be the empirical risk of $f_{\bm \theta}$ measured on $\mathcal{Z}$, where $\ell: \mathcal{Y} \times \mathcal{Y} \rightarrow \mathbb{R}^+$ is the loss function;
$\hat{\bm \theta} = \argmin_{\bm \theta} \mathcal{L}_{\mathcal{Z}, \bm \theta} $ and $\hat{\bm \theta}_{-i} = \argmin_{\bm \theta} \mathcal{L}_{\mathcal{Z}_{-i}, \bm \theta}$ be the optimal parameters of the model $f_{\bm \theta}$ trained on $\mathcal{Z}$ and $\mathcal{Z}_{-i}$.
In this paper, $f_{\bm \theta}$ is a deep network and $\hat{\bm \theta}$ is found by training $f_{\bm \theta}$ with gradient descent.

\subsection{Influence function and variants}

The influence of a data point $\mathbf{z}^{(i)}$ on another data point $\mathbf{z}^{(j)}$ is defined as 
\begin{align}
s^{(ij)} = \ell(\mathbf{z}^{(j)}; \hat{\bm \theta}_{-i}) - \ell(\mathbf{z}^{(j)}; \hat{\bm \theta})
\end{align}
$s^{(ij)} < 0$ means that removing $\mathbf{z}^{(i)}$ decreases the loss at $\mathbf{z}^{(j)}$.
In other words, $s^{(ij)} < 0$ means that $\mathbf{z}^{(i)}$ is harmful to $\mathbf{z}^{(j)}$.
The more negative $s^{(ij)}$ is, the more harmful $\mathbf{z}^{(i)}$ is to $\mathbf{z}^{(j)}$.
Averaging this influence score over a dataset $\mathcal{Z}'$ gives the influence of $\mathbf{z}^{(i)}$ on $\mathcal{Z}'$
\begin{align}
s^{(i)} = \frac{1}{\abs{\mathcal{Z}'}} \sum_{\mathbf{z}^{(j)} \in \mathcal{Z}'} s^{(ij)} \label{eqn:ifAverage}
\end{align}
$s^{(i)}$ is more stable than $s^{(ij)}$ and is commonly used in anomalous data detection \cite{cohen2020detecting, dau2022towards}.
Naive computation of $s^{(ij)}$ requires retraining $f_{\bm \theta}$ on $\mathcal{Z}_{-i}$.
\citet{koh2017understanding} used first and second order derivatives to quickly estimate $s^{(ij)}$ without retraining the model $f_{\bm \theta}$ on $\mathcal{Z}_{-i}$
\begin{align}
s^{(ij)} &\approx IF(\mathbf{z}^{(i)}, \mathbf{z}^{(j)}) \nonumber \\
&\approx \frac{1}{n} \nabla_{\hat{\bm \theta}} \ell(\mathbf{z}^{(i)}; \hat{\bm \theta})^\top H_{\hat{\bm \theta}}^{-1} \nabla_{\hat{\bm \theta}} \ell(\mathbf{z}^{(j)}; \hat{\bm \theta}) \label{eqn:if}
\end{align}
where $H_{\hat{\bm\theta}}$ is the Hessian at $\hat{\bm\theta}$.
Exact computation of $H^{-1}_{\hat{\bm \theta}}$ is intractable for modern networks.
\citet{koh2017understanding} developed a fast algorithm for estimating  $H_{\hat{\bm \theta}}^{-1} \nabla_{\hat{\bm \theta}} \ell(\mathbf{z}^{(j)}; \hat{\bm \theta})$ and used only the derivatives w.r.t.~the last layer's parameters to improve the algorithm's speed.
%\citet{basu2021influence} found that this approximation is a source of the instability of IF.
\citet{charpiat2019input} proposed gradient dot product (GD) and gradient cosine similarity (GC) as faster alternatives to IF.
\citet{pruthi2020estimating} argued that the influence can be better approximated by accumulating it through out the training process (TracIn).
The formula for IFs are summarized in Tab.~\ref{tab:ifs} in Appendix \ref{appx:formula}.

IFs can be viewed as measures of the similarity between the gradients of two data points.
The intuition of IFs is that gradients of harmful examples are dissimilar from that of normal examples.
%Influence functions considered in this paper is summerized in Tab.~\ref{tab:ifs}.

\subsection{Influence functions for error detection}

%IFs are a powerful tool for detecting anomalous data points.
%Although in this paper we focus on the error detection problem, our discussion and algorithm apply to other detection problems as well.

There are many kinds of noisy data such as outlier, mislabeled, or ambiguous data, that could have bad effects on the model.\footnote{We note that there might be mislabeled/ambiguous/outlier data points that do not have bad effects on the model. In this work, we are interested in detecting and removing/correcting data points with bad effects.}
\citet{beyer2020are} showed that a significant portion of the ImageNet \cite{deng2009imagenet} are mislabeled or have ambiguous labels.
For brevity, we call these data points errors.
Given a noisy dataset $\mathcal{Z}$ and we want to identify erroneous data points in $\mathcal{Z}$.

\citet{cohen2020detecting, dau2022towards} used IFs to detect adversarial and erroneous examples in classification datasets.
They used IFs to measure the influence of each data point $\mathbf{z} \in \mathcal{Z}$ on $\mathcal{Z}'$, a set of clean test data points. 
For the error detection task, data points in $\mathcal{Z}$ are ranked by how harmful they are to $\mathcal{Z}'$.
Most harmful data points are re-examined by human or are removed from $\mathcal{Z}$ (Alg.~\ref{alg:simErr} in Appendix \ref{appx:formula}).
In this paper, we focus on the error detection problem but IFs and IFs-class can be used to detect other kinds of anomalous data.
%In this paper, we introduce IFs-class, a stabilized version of IFs that can be used in detection algorithms.
%We extend the use IFs to sequential classification problems such as NER and PoS tagging.

%
%Alg.~\ref{alg:simErr} \cite{dau2022towards} uses IFs to measure the influence of a data point $\mathbf{z} \in \mathcal{Z}$ on a set of clean data points $\mathcal{Z}'$.
%If $\mathbf{z}$ has a negative influence on $\mathcal{Z}'$ then it is likely an error.
%Alg.~\ref{alg:simErr} ranks the data points in $\mathcal{Z}$ by how harmful they are.
%The most harmful data points are removed from the dataset or are re-labeled by human.
%\citet{dau2022towards} showed that models trained on the cleaned dataset have better performance than model trained on the original dataset.

